LED: A Dataset for Life Event Extraction from Dialogs

Lifelogging has gained more attention due to its wide applications, such as personalized recommendations or memory assistance. The issues of collecting and extracting personal life events have emerged. People often share their life experiences with others through conversations. However, extracting life events from conversations is rarely explored. In this paper, we present Life Event Dialog, a dataset containing fine-grained life event annotations on conversational data. In addition, we initiate a novel conversational life event extraction task and differentiate the task from the public event extraction or the life event extraction from other sources like microblogs. We explore three information extraction (IE) frameworks to address the conversational life event extraction task: OpenIE, relation extraction, and event extraction. A comprehensive empirical analysis of the three baselines is established. The results suggest that the current event extraction model still struggles with extracting life events from human daily conversations. Our proposed life event dialog dataset and in-depth analysis of IE frameworks will facilitate future research on life event extraction from conversations.

==> tables/model_constraints.tex <==
\begin{table*}[!htb]
    \centering
    \hspace{-1cm}
    \small
    \begin{tabular}{c|ccccl}
        Model & \thead{Implicit\\Evt} & \thead{No\\Evt} & \thead{No Obj\\Evt} & \thead{Use\\Coref} & Predicate \\\midrule
        OpenIE & \xmark & \cmark & \xmark & \xmark & Toks \\
        REBEL & \cmark & \xmark & \cmark & \xmark & Toks, Types \\
        DyGIE++ & \xmark & \xmark & \cmark & \cmark & Toks, Types \\
    \end{tabular}
    \caption{This table shows whether the model is able to predict implicit events, no event, or events without objects; if the model can make use of coreference information; and list the form of predicates, Tokens (Toks) and/or Event Type (Types), the model can take.}
    \label{tab:model_constraints}
\end{table*}

==> tables/results_DyGIE.tex <==
\begin{table*}[!hbt]
    \centering
    \small
    \begin{tabular}{lcccccccc|ccl}
        \toprule
        \multicolumn{1}{c}{\multirow{2}{*}{Event Type}} & \multicolumn{4}{c}{Validation} & \multicolumn{7}{c}{Test} \\
        \cmidrule(lr){2-5}\cmidrule(l){6-12}
        & T-ID & T-C & A-ID & A-C & T-ID & T-C & A-ID & A-C & ET-C & S-ID & \multicolumn{1}{c}{O-ID} \\
        \midrule
        \textit{Verb} & - & - & - & - & - & - & - & - & 44.8 & 37.2 & 14.5 / 46.2 / 9.2 \\
        \midrule
        \textit{Class} & 55.2 & 51.1 & 43.2 & 41.8 & 48.6 & 40.4 & 27.9 & 27.9 & 37.1 & 30.2 & 14.5 / 55.2 / 10.3 \\
        \quad+ coref & 54.6 & 45.1 & 39.9 & 39.9 & 57.7 & 31.2 & 20.9 & 20.9 & 28.0 & 19.3 & 12.7 / 19.3 / 9.9 \\
        \midrule
        \textit{Frame} & 49.3 & 35.3 & 31.6 & 30.5 & 50.5 & 33.0 & 21.6 & 21.6 & 32.0 & 25.1 & 14.4 / 46.3 / 11.5 \\
        \quad+ coref & 46.4 & 31.8 & 30.0 & 27.7 & 39.9 & 22.4 & 18.2 & 18.2 & 19.2 & 19.2 & \textcolor{white}{0}7.1 / 74.2 / 14.9 \\
        \bottomrule
    \end{tabular}
    \caption{Results from EE framework. Left: Original metrics, Trigger (T) and Arguments's (A) identification (ID) and classification (C). Right: our lenient metrics, Event Type Classification (ET-C), Subject Identification (S-ID), and Object Identification (O-ID) (F1/Bert Score/BLEU). }
    \label{tab:results_dygie}
\end{table*}


==> tables/results_OpenIE_Rebel.tex <==
\begin{table*}[!htb]
    \centering
    \small
    \begin{tabular}{cccccccc|ccl}
    \toprule
        \multirow{2}{*}{Framework} & \multirow{2}{*}{\thead{Event\\Type}} & \multicolumn{3}{c}{Validation} & \multicolumn{6}{c}{Test} \\
        \cmidrule(lr){3-5}\cmidrule(l){6-11}
        &  & P & R & F1 & P & R & F1 & ET-C & S-ID & \multicolumn{1}{c}{O-ID} \\\midrule
        OpenIE & \textit{Verb} & 3.6 & 5.7 & 4.4 & 5.6 & 8.8 & 6.8 & 22.6 & 21.1 & 7.9 / 33.5 / 2.0 \\
        \midrule
        \multirow{3}{*}{RE} & \textit{Verb} & 54.2 & 36.9 & 43.9 & 40.7 & 24.7 & 30.8 & 52.8 & 47.5 & 27.9 / 65.1 / 17.0 \\
        & \textit{Class} & 47.1 & 33.6 & 39.2 & 41.5 & 26.0 & 32.0 & 51.8 & 47.9 & 27.6 / 64.1 / 16.2 \\
        & \textit{Frame} & 43.6 & 34.9 & 38.8 & 29.4 & 19.2 & 23.2 & 35.2 & 29.7 & 17.7 / 60.9 / 16.9 \\
    \bottomrule
    \end{tabular}
    \caption{OpenIE and RE frameworks evaluated by the original metrics (left: P, R, F1 (strict evaluation)) and our metrics (right: ET-C F1, S-ID F1, O-ID F1/Bert Score/BLEU). }
    \label{tab:results_triple}
\end{table*}


==> tables/results_falseEvents.tex <==
\begin{table}[t]
\centering
\small
\resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{\thead{Event\\Type}} &  \multirow{2}{*}{Model} &  ET &  S &  \multicolumn{3}{c}{O} \\\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-7}
        &   &  F1 & F1 & F1 & BS & BLEU \\ %\multicolumn{1}{c}{F1} &  \multicolumn{1}{c}{F1} &  \multicolumn{1}{c}{F1} &  \multicolumn{1}{c}{BS} &  \multicolumn{1}{c}{BLEU} \\
        \midrule
        \multirow{2}{*}{\textit{Token}} & E & 52.8 & 47.5 & 27.9 & 65.1 & 17.0 \\
         & E $+$ I & 31.7 & 27.3 & 17.8 & 56.3 & 16.2 \\
        \midrule
        \multirow{2}{*}{\textit{Verb}} & E & 51.8 & 47.9 & 27.6 & 64.1 & 16.2 \\
         & E $+$ I & 40.2 & 37.0 & 18.7 & 59.9 & 13.6 \\
        \midrule
        \multirow{2}{*}{\textit{Frame}} & E & 35.2 & 29.7 & 17.7 & 60.9 & 16.9 \\
         & E $+$ I & 31.9 & 26.2 & 15.2 & 60.9 & 15.7 \\
    \bottomrule
    \end{tabular}
}
\caption{}
\label{tab:results_false}
\end{table}

==> tables/top10_frame-verb.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l|l}
        Frame (\%) & Class (Count) \\
        \midrule
        Statement (6.1) & 
        (tell, 69), (talk, 26), (say, 9) \\ %, (introduce, 7), (speak, 5), (explain, 5), (inform, 4), (report, 2), (convey, 2), (repeat, 1) \\
        Perception (5.3) & 
        (hear, 60), (see, 47), (experience, 4) \\ %, (look, 1) \\
        Motion (3.8) & 
        (go, 57), (come, 14), (head, 4) \\ %, (travel, 3), (move, 1), (follow, 1) \\
        Request (3.2) & (invite, 24), (order, 14), (request, 11) \\ %, (ask, 9), (apply, 6), (call, 3), (be invite, 2) \\
        Ingestion (3.2) & 
        (have, 30), (eat, 27), (drink, 7) \\ %, (have recover, 1), (eat much, 1), (take, 1), (have be fire, 1) \\
        Giving (3.1) & 
        (give, 47), (leave, 10), (serve, 3) \\ %, (get, 2), (pass, 2), (offer, 1), (tip, 1) \\
        Possession (3.0) & 
        (have, 53), (get, 10), (possess, 1) \\
        % not_selected (6.1\%) & 
        % (be, 8), (" m", 6), (dream, 4), (with, 3), (invite, 3), (interview, 2), (s, 2), (late, 2), (greet, 2), (apologize, 2) \\
        Bringing (2.5) & 
        (bring, 50), (get, 2), (take, 1) \\ %, (carry, 1) \\
        Acquaintance (2.4) & 
        (meet, 34), (see, 11), (meeting, 3) \\ %, (accompany, 2), (get together, 2) \\
        Receiving (2.3) & 
        (receive, 38), (get, 12)
    \end{tabular}
    \caption{This table shows the top 10 frame names, its percentage in the dataset, and the top 3 predicate classes and its count in each frame. Perception: Perception\_experience, Acquaintance: Make\_acquaintance}
    \label{tab:top10_frame_verb}
\end{table}

==> tables/top10_topic_eventTypes.tex <==
\begin{table*}[!htb]
    \centering
    \begin{tabular}{lrlrlrlrlrlr}
    \toprule
    \multicolumn{4}{c}{Relationship} & \multicolumn{4}{c}{Ordinary Life} & \multicolumn{4}{c}{Work} \\
    \cmidrule{1-4}\cmidrule(rl){5-8}\cmidrule{9-12}
    Frame   & \% &    Class & \% & Frame   & \% &    Class & \% & Frame   & \% &     Class & \% \\
    \cmidrule(r){1-2}\cmidrule(rl){3-4}\cmidrule(rl){5-6}\cmidrule(rl){7-8}\cmidrule(l){9-12}
    Perception & 7.9 & go & 7.7 & Perception & 4.7 & look & 4.9 & Statement & 11.3 & have & 4.6 \\
    Motion & 6.3 & hear & 4.8 & Statement & 4.6 & have & 4.1 & Possession & 3.9 & tell & 4.6 \\
    Statement & 6.0 & meet & 4.0 & Giving & 4.6 & give & 3.7 & Giving & 3.9 & work & 3.5 \\
    Acquaintance & 5.8 & invite & 3.7 & Ingestion & 4.2 & tell & 3.6 & Request & 3.2 & see & 2.8 \\
    Request & 4.3 & see & 3.6 & Bringing & 3.7 & bring & 3.6 & Employed & 3.0 & talk & 2.8 \\ 
    \midrule
    \multicolumn{4}{c}{Tourism} &  \multicolumn{4}{c}{Attitude \&  Emotion} &  \multicolumn{4}{c}{All} \\
    \cmidrule{1-4}\cmidrule(rl){5-8}\cmidrule{9-12}
    Frame   & \% &    Class & \% & Frame   & \% &    Class & \% & Frame   & \% &     Class & \% \\
    \cmidrule(r){1-2}\cmidrule(rl){3-4}\cmidrule(rl){5-6}\cmidrule(rl){7-8}\cmidrule(l){9-12}
    Motion & 5.4 & pay & 5.4 & Bringing & 8.9 & bring & 7.4 & Statement & 6.1 & have & 3.9 \\
Pay & 5.4 & go & 4.7 & Perception & 6.7 & have & 5.9 & Perception & 5.3 & go & 3.8 \\
Reserving & 5.0 & have & 3.9 & Ingestion & 5.2 & hear & 5.2 & Motion & 3.8 & tell & 3.5 \\
Suasion & 4.7 & change & 3.6 & Receiving & 5.2 & be & 3.7 & Request & 3.2 & hear & 2.8 \\
Perception & 4.3 & send & 3.6 & Possession & 4.4 & receive & 3.7 & Ingestion & 3.2 & see & 2.8 \\
    \bottomrule
    \end{tabular}%}
    \caption{Top 5 \textit{Frame} and \textit{Class} in each topic.}
    \label{tab:freq_event_types}
\end{table*}

==> tables/top10_topic_explicitness.tex <==
\begin{table*}[!htb]
    \centering
    \small
    \begin{tabular}{cc|cc|cc|cc|cc}
    \multicolumn{2}{c|}{Rel.} & \multicolumn{2}{c|}{Life} & \multicolumn{2}{c|}{Work} & \multicolumn{2}{c|}{Tour} & \multicolumn{2}{c}{Emo.} \\\cmidrule{1-10}
    Explicit & Implicit & Explicit & Implicit & Explicit & Implicit & Explicit & Implicit & Explicit & Implicit \\\midrule
    go & invite & have & give & have & work & go & pay & have & bring \\
    see & hear & look & receive & tell & study & have & hear & be & receive \\
    meet & eat & tell & pay & see & request & change & receive & bring & hear \\
    hear & receive & show & order & talk & buy & send & give & hear & borrow \\
    tell & go & bring & look & be & receive & check & call & buy & eat \\
    have & give & see & ask & get & change & tell & reserve & lend & wear \\
    get & bring & recommend & buy & call & notice & put & visit & know & have \\
    buy & refuse & try on & eat & ask & ask & book & appoint & send & travel \\
    watch & come & call & hear & leave & interview & recommend & travel & get & look \\
    say & lend & give & request & give & hear & bring & book & go & come \\
    \end{tabular}
    \caption{Top 10 explicit and implicit predicate classes by topic.}
    \label{tab:explicit_implicit_by_topic}
\end{table*}
